Reinforcing What the Student Has Learned: Teacher-Guided On-Policy Distillation

On-policy distillation (OPD) improves language-model reasoning through dense teacher feedback on student-generated responses. We first observe an amplitude disparity in this feedback: on math reasoning responses, style-related positions exhibit 3.5 times the mean absolute teacher--student log-probability difference of mathematical positions. Scaling OPD updates by these discrepancies thus directs much of the update strength toward matching the teacher's expression. We instead take the student's own pretrained base as a reference: the student--base difference records the token preferences acquired during post-training and provides supervision that does not depend on the student's distance from the teacher. Building on this reference, we propose Student-Delta On-Policy Distillation (SD-OPD), which uses centered student--base differences as update coefficients, keeps each coefficient only when its sign agrees with centered teacher--student feedback, and recomputes the student signal every training round. Across 5 teacher--student configurations with Qwen3 students of 1.7B to 8B parameters, SD-OPD improves six-task mathematics average pass@1 (avg@16) over OPD by 7.76 to 10.37 percentage points. Code is available at https://github.com/aim-uofa/sd-opd.

==> tables/generalization_preference_rows.tex <==
% Source: analysis/outputs/generalization_analysis/student/summary.json
% Verified against preferences_per_question.csv; generated by draw/export_generalization_preferences.py
suppose & $+2.617$ & 57.6 \\
try & $+2.671$ & 21.9 \\
strategy & $+2.267$ & 23.5 \\
idea & $+2.246$ & 75.8 \\
straightforward & $-1.188$ & 84.2 \\
simplicity & $-0.505$ & 55.7 \\

